Microstructural Characterization and Mechanical Property Evaluation of High Nitrogen Martensitic Stainless Steel Subjected to Heat Treatment

The High Nitrogen Martensitic Stainless Steel (HNMS) was subjected to three different austenitizing cycles of 1050$^\circ$C, 1075$^\circ$C and 1100$^\circ$C followed by subzero treatment at -70$^\circ$C. The fraction of retained austenite has been reduced after sub-zero treatment as revealed by microstructural evolution. The material was subsequently tempered at different temperatures ranging from 180$^\circ$C to 650$^\circ$C and the change in micro-structure, hardness, tensile strength and toughness were investigated after each heat treatment cycle. Optical microscopy, electron microscopy with EDS and X-Ray diffraction techniques were used to characterize the material. This has showed the constituents of microstructure were lath martensite, precipitated metal carbides of type $M_{23}C_6$, $M_7C_6$ and carbo-nitrides. Hardness, tensile testing and Charpy impact testing were carried to evaluate mechanical properties after the heat treatment which has showed the better mechanical properties for the samples solutionised at 1075$^\circ$C. Secondary hardening has been observed on tempering above 450$^\circ$C which can be attributed to the precipitation of secondary phase inter-metallic compounds. Hardness attains a peak value at peculiar temperature range after which it decreases on further tempering which is most likely because of the loss of coherency of the precipitates with the metal matrix. This has been further confirmed by the XRD of the specimens before and after tempering. The study stablishes the structure-property correlation of HNMS for different heat treatment cycles. The results indicate that a good combination of hardness and strength can be achieved after solutionizing at 1075$^\circ$C followed by double tempering at 525$^\circ$C.

==> bibfile.tex <==
@article{fan2012effects,
  title={Effects of heat treatment and nitrogen on microstructure and mechanical properties of 1Cr12NiMo martensitic stainless steel},
  author={Fan, Ruicheng and Gao, Ming and Ma, Yingche and Zha, Xiangdong and Hao, Xianchao and Liu, Kui},
  journal={Journal of Materials Science \& Technology},
  volume={28},
  number={11},
  pages={1059--1066},
  year={2012},
  publisher={Elsevier}
}

@inproceedings{girodin2002characterisation,
  title={Characterisation of the XD15N high nitrogen martensitic stainless steel for aerospace bearings},
  author={Girodin, D and Manes, L and Moraux, JY and De Monicault, JM},
  booktitle={Proceedings de 4th International Conference on Launcher Technology" Space Launcher Liquid Propulsion},
  year={2002}
}

@article{gingell1997carbide,
  title={Carbide precipitation in some secondary hardened steels},
  author={Gingell, AD B and Bhadeshia, HKD H and Jones, DG and Mawella, KJ A},
  journal={Journal of Materials Science},
  volume={32},
  number={18},
  pages={4815--4820},
  year={1997},
  publisher={Springer}
}


@inproceedings{hucklenbroich1999high,
  title={High nitrogen martensitic steel for critical components in aviation},
  author={Hucklenbroich, I and Stein, G and Chin, H and Trojahn, W and Streit, E},
  booktitle={Materials science forum},
  volume={318},
  pages={161--166},
  year={1999},
  organization={Trans Tech Publ}
}


@article{nykiel2014transformations,
  title={Transformations of carbides during tempering of D3 tool steel},
  author={Nykiel, Tadeusz and Hryniewicz, Tadeusz},
  journal={Journal of materials engineering and performance},
  volume={23},
  number={6},
  pages={2050--2054},
  year={2014},
  publisher={Springer}
}


@article{byrnes1987nitrogen,
  title={Nitrogen strengthening of a stable austenitic stainless steel},
  author={Byrnes, MLG and Grujicic, M and Owen, WS},
  journal={Acta Metallurgica},
  volume={35},
  number={7},
  pages={1853--1862},
  year={1987},
  publisher={Elsevier}
}

@article{speidel1992high,
  title={High nitrogen stainless steels in chloride solutions},
  author={Speidel, Markus O and Pedrazzoli, Ruth M},
  journal={Materials performance},
  volume={31},
  number={9},
  pages={59--61},
  year={1992}
}

@inproceedings{hucklenbroich1999high,
  title={High nitrogen martensitic steel for critical components in aviation},
  author={Hucklenbroich, I and Stein, G and Chin, H and Trojahn, W and Streit, E},
  booktitle={Materials science forum},
  volume={318},
  pages={161--166},
  year={1999},
  organization={Trans Tech Publ}
}


@article{ojima2008origin,
  title={Origin of the enhanced hardness of a tempered high-nitrogen martensitic steel},
  author={Ojima, M and Ohnuma, M and Suzuki, J and Ueta, S and Narita, S and Shimizu, T and Tomota, Y},
  journal={Scripta Materialia},
  volume={59},
  number={3},
  pages={313--316},
  year={2008},
  publisher={Elsevier}
}


@article{zhu2014effect,
  title={Effect of Ni on the stability of retained austenite and mechanical properties for TRIP steels containing vanadium},
  author={Zhu, Naqiong and Wu, Qihao and He, Yanlin and Lu, Xiaogang and Li, Lin and Hu, Pengfei},
  journal={steel research international},
  volume={85},
  number={2},
  pages={143--154},
  year={2014},
  publisher={Wiley Online Library}
}


@article{krishna2015effect,
  title={Effect of heat treatment on the microstructure and hardness of 17Cr-0.17 N-0.43 C-1.7 Mo martensitic stainless steel},
  author={Krishna, S Chenna and Gangwar, Narendra Kumar and Jha, Abhay K and Pant, Bhanu and George, Koshy M},
  journal={Journal of Materials Engineering and Performance},
  volume={24},
  number={4},
  pages={1656--1662},
  year={2015},
  publisher={Springer}
}


@article{krauss1971morphology,
  title={The morphology of martensite in iron alloys},
  author={Krauss, G and Marder, AR},
  journal={Metallurgical Transactions},
  volume={2},
  number={9},
  pages={2343--2357},
  year={1971},
  publisher={Springer}
}

@article{bhadeshia1997martensite,
  title={Martensite and bainite in steels: transformation mechanism \& mechanical properties},
  author={Bhadeshia, HKDH},
  journal={Le Journal de Physique IV},
  volume={7},
  number={C5},
  pages={C5--367},
  year={1997},
  publisher={EDP sciences}
}


@article{lee2009reverse,
  title={Reverse transformation mechanism of martensite to austenite in a metastable austenitic alloy},
  author={Lee, Seok-Jae and Park, Yong-Min and Lee, Young-Kook},
  journal={Materials Science and Engineering: A},
  volume={515},
  number={1-2},
  pages={32--37},
  year={2009},
  publisher={Elsevier}
}


@article{lee2009reverse,
  title={Reverse transformation mechanism of martensite to austenite in a metastable austenitic alloy},
  author={Lee, Seok-Jae and Park, Yong-Min and Lee, Young-Kook},
  journal={Materials Science and Engineering: A},
  volume={515},
  number={1-2},
  pages={32--37},
  year={2009},
  publisher={Elsevier}
}

@article{fan2012effects,
  title={Effects of heat treatment and nitrogen on microstructure and mechanical properties of 1Cr12NiMo martensitic stainless steel},
  author={Fan, Ruicheng and Gao, Ming and Ma, Yingche and Zha, Xiangdong and Hao, Xianchao and Liu, Kui},
  journal={Journal of Materials Science \& Technology},
  volume={28},
  number={11},
  pages={1059--1066},
  year={2012},
  publisher={Elsevier}
}

@article{isfahany2011effect,
  title={The effect of heat treatment on mechanical properties and corrosion behavior of AISI420 martensitic stainless steel},
  author={Isfahany, A Nasery and Saghafian, H and Borhani, Gh},
  journal={Journal of alloys and compounds},
  volume={509},
  number={9},
  pages={3931--3936},
  year={2011},
  publisher={Elsevier}
}

@article{pant2013studies,
  title={Studies towards development of laser peening technology for martensitic stainless steel and titanium alloys for steam turbine applications},
  author={Pant, BK and Sundar, R and Kumar, Harish and Kaul, R and Pavan, AHV and Ranganathan, K and Bindra, KS and Oak, SM and Kukreja, LM and Prakash, Raghu V and others},
  journal={Materials Science and Engineering: A},
  volume={587},
  pages={352--358},
  year={2013},
  publisher={Elsevier}
}
